ShEF: Shielded Enclaves for Cloud FPGAs

FPGAs are now used in public clouds to accelerate a wide range of applications, including many that operate on sensitive data such as financial and medical records. We present ShEF, a trusted execution environment (TEE) for cloud-based reconfigurable accelerators. ShEF is independent from CPU-based TEEs and allows secure execution under a threat model where the adversary can control all software running on the CPU connected to the FPGA, has physical access to the FPGA, and can compromise the FPGA interface logic of the cloud provider. ShEF provides a secure boot and remote attestation process that relies solely on existing FPGA mechanisms for root of trust. It also includes a Shield component that provides secure access to data while the accelerator is in use. The Shield is highly customizable and extensible, allowing users to craft a bespoke security solution that fits their accelerator's memory access patterns, bandwidth, and security requirements at minimum performance and area overheads. We describe a prototype implementation of ShEF for existing cloud FPGAs, map ShEF to a performant and secure storage application, and measure the performance benefits of customizable security using five additional accelerators.

==> Makefile <==
TEX_SOURCES=$(shell ls *.tex)
ALL_FIGS=$(shell find figures -type f)

all: main.pdf

view: main.pdf
	open main.pdf

RERUN=egrep -q '(^LaTeX Warning:|\(natbib\)).* Rerun' main.log

main.pdf: ${TEX_SOURCES} figures
	pdflatex -interaction=nonstopmode main.tex
	bibtex -min-crossrefs=1000 main 
	pdflatex -interaction=nonstopmode main.tex
	pdflatex -interaction=nonstopmode main.tex
	while ( $(RERUN) ); do pdflatex main.tex; done

figures: $(ALL_FIGS)

clean:
	rm -rf *.aux *.bbl *.blg *.log *.out *.synctex.gz *.fls *.fdb_latexmk main.pdf

# The following target is useful for debugging Makefiles; it
# prints the value of a make variable.
print-%:
	@echo $* = $($*)

.PHONY: figures clean all view

.PRECIOUS:
.SECONDARY:


==> fig-f1.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.90\linewidth]{figs/f1.pdf}
\caption{\small The AWS EC2 F1 development process.}
\label{fig:f1-dev}
\end{figure}

==> implementation.tex <==
\section{Implementation}\label{sec:implementation}

We prototyped \SystemName for the Xilinx UltraScale+  FPGA used by AWS F1. Since \SystemName only relies on the AES key storage and an SPB, it can also be implemented on Intel FPGAs. Since we are not allowed to deploy our secure boot process on AWS, we used a local UltraScale+ Ultra96 FPGA board~\cite{u96} to develop and test it. We deployed various Shield configurations with accelerators on AWS F1 instances in order to evaluate performance (assuming successful boot and attestation).  



As mentioned in Section~\ref{sec:architecture}, the root-of-trust is a set of two keys, one AES key embedded in the secure storage and an asymmetric key in the encrypted firmware.
We provisioned an AES key and programmed it into the Ultra96 e-fuses.
The Ultra96 boot process first executes out of BootROM on the SPB with exclusive access to the cryptographic hardware and the programming ports.
We embedded the private device key into the firmware and encrypted it with the AES device key.
The firmware, after decryption, is loaded onto another hardened processor called the platform management unit (PMU). We boot the Security Kernel on a dedicated Cortex-R5 core, which runs solely from dedicated on-chip memory. %
The Security Kernel communicates with the SPB via a dedicated IPI interface to access cryptographic hardware to generate attestation reports, and runs on the R5 core continuously, monitoring FPGA programming and debug ports.

We implemented the Shield as portable RTL code in the 2019.2 version of Xilinx tools that can target any Xilinx FPGA.
The Shield interfaces with the host program via a \SystemName runtime library, which links against the Xilinx runtime (XRT) that provides drivers, libraries, and management tools for controlling the accelerator.

Developers can use standard libraries and frameworks such as OpenCL and SDAccel to develop and control their accelerator in conjunction with the software runtime.
XRT and the host user program are not in the trusted computing base (TCB).
Users who wish to integrate \SystemName with other trusted code, such as an enclave running on the  CPU, can  leverage the host runtime as a proxy to create a secure channel.
This allows developers to specialize their trusted application to take advantages of both \SystemName and traditional TEEs (e.g. SGX). 

We measured the full end-to-end \SystemName workflow on the Ultra96 board, and observed that the boot process, from power-on to bitstream loading, completes in 5.1 seconds.
This is relatively small compared to the commonly-observed 40+ second boot times of CSP VM instances~\cite{gce-boot-times, boot-times}, plus the $\approx$6.2 second bitstream loading times we observe on F1.




==> tbl-tee-reqs.tex <==
\begin{table}[]
\begin{tabular}{l}
\hline
TEE Requirements          \\ \hline
Hardware Root of Trust    \\
Secure Boot               \\
Remote Attestation        \\
Secure Storage and I/O    \\
Isolated Execution        \\
Flexibility               \\
Bitstream Confidentiality \\ \hline
\end{tabular}
\end{table}
